Finding agreement cherry-reduced subnetworks in level-1 networks

Phylogenetic networks are increasingly being considered as better suited to represent the complexity of the evolutionary relationships between species. One class of phylogenetic networks that has received a lot of attention recently is the class of orchard networks, which is composed of networks that can be reduced to a single leaf using cherry reductions. Cherry reductions, also called cherry-picking operations, remove either a leaf of a simple cherry (sibling leaves sharing a parent) or a reticulate edge of a reticulate cherry (two leaves whose parents are connected by a reticulate edge). In this paper, we present a fixed-parameter tractable algorithm to solve the problem of finding a maximum agreement cherry-reduced subnetwork (MACRS) between two rooted binary level-1 networks. This is first exact algorithm proposed to solve the MACRS problem. As proven in earlier work, there is a direct relationship between finding an MACRS and calculating a distance based on cherry operations. As a result, the proposed algorithm also provides a distance that can be used for the comparison of level-1 networks.

==> figures/b-comp.tex <==
\begin{figure}
    \centering
    \begin{tikzpicture}
        \coordinate (R) at (0,0);
        \coordinate (r) at (0,-1);
        \coordinate (A) at (-1,-2);
        \coordinate (B) at (1,-2);
        \draw (R) -- (r);
        \draw (A) -- (r) -- (B);
        \coordinate (g) at (0.5,-3);
        \draw (B) -- (g);
        \coordinate (G) at (1.5,-3);
        \draw (B)--(G);
         \foreach \v in {r,A,B,G} {
            \node[circle,draw,inner sep=0.5mm,fill=black] at (\v) {};
        }
        \foreach \l/\angle in {g/north east} {
            \node[anchor=\angle,circle,draw,inner sep=0.5mm] at (\l) {};
        }
    \end{tikzpicture}
    \caption{caption}
    \label{fig:my_label}
\end{figure}
